Physics-Informed Optical Kernel Regression Using Complex-valued Neural Fields

Lithography is fundamental to integrated circuit fabrication, necessitating large computation overhead. The advancement of machine learning (ML)-based lithography models alleviates the trade-offs between manufacturing process expense and capability. However, all previous methods regard the lithography system as an image-to-image black box mapping, utilizing network parameters to learn by rote mappings from massive mask-to-aerial or mask-to-resist image pairs, resulting in poor generalization capability. In this paper, we propose a new ML-based paradigm disassembling the rigorous lithographic model into non-parametric mask operations and learned optical kernels containing determinant source, pupil, and lithography information. By optimizing complex-valued neural fields to perform optical kernel regression from coordinates, our method can accurately restore lithography system using a small-scale training dataset with fewer parameters, demonstrating superior generalization capability as well. Experiments show that our framework can use 31% of parameters while achieving 69$\times$ smaller mean squared error with 1.3$\times$ higher throughput than the state-of-the-art.

==> doc/res/aerial.tex <==
% \begin{table}[tb!]
%   \centering
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{.1}
%   \begin{tabular}{lccccc}
%       \midrule
%       (a) B1   & \includegraphics[width=.15\linewidth,valign=m]{res/ibm_mask}   & \includegraphics[width=.15\linewidth,valign=m]{res/ibm_aerial_gt}   & \includegraphics[width=.15\linewidth,valign=m]{res/ibm_aerial_nitho}   & \includegraphics[width=.15\linewidth,valign=m]{res/ibm_aerial_fno}   & \includegraphics[width=.15\linewidth,valign=m]{res/ibm_resist_nitho} \\ \midrule
%       (b) B2m  & \includegraphics[width=.15\linewidth,valign=m]{res/b2m_mask}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2m_aerial_gt}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2m_aerial_nitho}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2m_aerial_fno}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2m_resist_nitho} \\ \midrule
%       (c) B2v  & \includegraphics[width=.15\linewidth,valign=m]{res/b2v_mask}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2v_aerial_gt}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2v_aerial_nitho}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2v_aerial_fno}   & \includegraphics[width=.15\linewidth,valign=m]{res/b2v_resist_nitho} \\ \midrule
%       & Mask & Aerial G.T. & Nitho &  Resist G.T. & Nitho \\
%   \end{tabular}
%   \captionof{figure}{Visualization of the results of Nitho in aerial and resist stage.}
%   \label{fig:vis_masks}
% \end{table}

==> doc/res/nelitho_unseen.tex <==
% \begin{table}[htbp]
%   \centering
%   \caption{Test on unseen dataset.}
%   % \setlength{\tabcolsep}{3pt}
% 	\renewcommand{\arraystretch}{1.1}
%   \begin{tabular}{ll|ccc}
%   \toprule
%   Train on & Test on & MSE ($\times 10^{-5}$)           & ME ($\times 10^{-2}$) & PSNR (dB)  \\ \midrule
%   B1                        & B1opc                    & 80 (10)        &         &              \\
%   B2m                       & B2v                      &                &         &              \\
%   B2v                       & B2m                      &                &         &              \\ \midrule
%   \multicolumn{2}{c|}{Average}                         &                &         &               \\
%   \bottomrule
%   \end{tabular}
% \end{table}

==> figs/pgfplot/tnum/tnum.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

  \definecolor{darkgray176}{RGB}{176,176,176}
  \definecolor{darkslateblue10661154}{RGB}{106,61,154}
  \definecolor{forestgreen5116044}{RGB}{51,160,44}
  \definecolor{lightgray204}{RGB}{204,204,204}
  \definecolor{lightslategray127115175}{RGB}{127,115,175}
  \definecolor{steelblue31120180}{RGB}{31,120,180}
  
  \begin{axis}[
  legend cell align={left},
  legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,0.92)}, draw=lightgray204},
  tick align=outside,
  tick pos=left,
  x grid style={darkgray176},
  xlabel={Training set percentage},
  xmin=-0.02375, xmax=1.04875,
  xtick style={color=black},
  y grid style={darkgray176},
  ylabel={PSNR},
  ymin=30.74, ymax=50.32,
  ytick style={color=black}
  ]
  \addplot [
    draw=lightslategray127115175,
    fill=lightslategray127115175,
    forget plot,
    mark=*,
    only marks,
    opacity=0.8
  ]
  table{%
  x  y
  0.025 40.51
  0.05 43.73
  0.075 43.41
  0.125 44.03
  0.175 45.33
  0.25 48.4
  0.375 48.35
  0.5 49.37
  0.75 49.43
  1 49.28
  };
  \addplot [
    draw=lightslategray127115175,
    fill=lightslategray127115175,
    forget plot,
    mark=*,
    only marks,
    opacity=0.8
  ]
  table{%
  x  y
  0.025 33.51
  0.05 35.63
  0.075 37.28
  0.125 36.08
  0.175 38.25
  0.25 38.5
  0.375 39.4
  0.5 39.07
  0.75 41.1
  1 40.74
  };
  \addplot [
    draw=lightslategray127115175,
    fill=lightslategray127115175,
    forget plot,
    mark=*,
    only marks,
    opacity=0.8
  ]
  table{%
  x  y
  0.025 31.63
  0.05 33.02
  0.075 33.75
  0.125 33.48
  0.175 34.32
  0.25 34.75
  0.375 34.28
  0.5 34.36
  0.75 34.82
  1 34.65
  };
  \addplot [very thick, steelblue31120180]
  table {%
  0.025 40.51
  0.05 43.73
  0.075 43.41
  0.125 44.03
  0.175 45.33
  0.25 48.4
  0.375 48.35
  0.5 49.37
  0.75 49.43
  1 49.28
  };
  \addlegendentry{Nitho}
  \addplot [very thick, darkslateblue10661154]
  table {%
  0.025 33.51
  0.05 35.63
  0.075 37.28
  0.125 36.08
  0.175 38.25
  0.25 38.5
  0.375 39.4
  0.5 39.07
  0.75 41.1
  1 40.74
  };
  \addlegendentry{DOINN}
  \addplot [very thick, forestgreen5116044]
  table {%
  0.025 31.63
  0.05 33.02
  0.075 33.75
  0.125 33.48
  0.175 34.32
  0.25 34.75
  0.375 34.28
  0.5 34.36
  0.75 34.82
  1 34.65
  };
  \addlegendentry{TEMPO}
  \end{axis}
  
  \end{tikzpicture}
  
